Synthesis of Data Completion Scripts using Finite Tree Automata

In application domains that store data in a tabular format, a common task is to fill the values of some cells using values stored in other cells. For instance, such data completion tasks arise in the context of missing value imputation in data science and derived data computation in spreadsheets and relational databases. Unfortunately, end-users and data scientists typically struggle with many data completion tasks that require non-trivial programming expertise. This paper presents a synthesis technique for automating data completion tasks using programming-by-example (PBE) and a very lightweight sketching approach. Given a formula sketch (e.g., AVG($?_1$, $?_2$)) and a few input-output examples for each hole, our technique synthesizes a program to automate the desired data completion task. Towards this goal, we propose a domain-specific language (DSL) that combines spatial and relational reasoning over tabular data and a novel synthesis algorithm that can generate DSL programs that are consistent with the input-output examples. The key technical novelty of our approach is a new version space learning algorithm that is based on finite tree automata (FTA). The use of FTAs in the learning algorithm leads to a more compact representation that allows more sharing between programs that are consistent with the examples. We have implemented the proposed approach in a tool called DACE and evaluate it on 84 benchmarks taken from online help forums. We also illustrate the advantages of our approach by comparing our technique against two existing synthesizers, namely PROSE and SKETCH.

==> construction.tex <==
\section{Representation construction}

In this section, we present the algorithm for constructing the program set that represents all conditional-free programs for an example. 


==> limitations.tex <==
\section{Limitations and Future Work}

We plan to apply the techniques proposed in this paper to more scenarios other than data completion. 
One current limitation of \tool is that the predicate language only contains conjunctive string equalities (up to size $3$). 
Although this is not a serious problem in the domain of data completion, we envision it would be necessary to improve the predicate language expressiveness by extending its vocabulary to support more features, such as substring matching. 
As a result, this might lead to potential scalability issues, which we plan to address by designing predicate learning algorithms or using symbolic encoding. 
Another idea we plan to work on is to improve the top-level synthesis algorithm, since the worst-case running time is $\mathcal{O}(n^m)$ in the number of examples $n$ and the number of branches $m$ in the learned program. In the domain of data completion, this is not a problem due to the effectiveness of a ranking algorithm. However, for situations where it is hard to predicate a correct program with few examples, the efficiency of the synthesis algorithm would be critical for improving the scalability of the whole system. 


==> overview.tex <==
\section{Algorithm overview}

In this section, we present an overview of the synthesis algorithm. 
We first illustrate how it works on a simple example, then we explain how to generalize the algorithm to learn programs in the full $\dsl$. 

\subsection{A simple example}

\begin{example}[Conditional LOCF]
$\david$ had a dataset with some missing values as shown in \figref{locfseq}.
He wanted to replace each missing value by the previous non-missing value in the same column, and if that does not exist, the next non-missing value in that column is used.
\exlabel{locfseq} 
\end{example}


\begin{figure}
\centering
\includegraphics[scale=0.6]{figs/locfseq.png}
\caption{Conditional LOCF.}
\figlabel{locfseq}
\end{figure}


$\tool$ first takes an example table, and a sketch for calculating the missing value. 
In this case, the example table given by $\david$ is the first five columns of the original table, and the sketch is the identity function $\t{ID}(\hole)$. 

\underline{\textit{Iteration $1$}:}
$\david$ gave the first example equation $(5,3) \assign \texttt{ID}((4,3))$ for calculating the value in cell at position $(5,3)$. 
$\tool$ translates this equation into an input-output example for the data extraction task, which is $(5,3) \mapsto (4,3)$. 
It then constructs an automaton $\progset_1$ in such a way that the initial state represents cell $(5,3)$, the final state represents cell $(4,3)$, and the strings accepted by $\progset_1$ represent all the conditional-free programs in the $\dsl$ that match the example. 
Then, $\tool$ returns the ``simplest'' one among all consistent programs as the answer to $\david$, say, $\getcell(\inputcell, \updir, 1, \lambda\startcell.\lambda\itercell. \true)$. 

With this program, $\david$ managed to fill some missing cells correctly, such as cells as positions $(6,4), (6,5), (2,5)$, but all the others are still missing. 

\underline{\textit{Iteration $2$:}}
$\david$ gave a second example equation for calculating the value of a cell that is still missing, say, $(7,5) \assign \texttt{ID}((5,5))$. 
$\tool$ translates this example equation into an example $(7,5) \mapsto (5,5)$, and then constructs an automaton $\progset_2$ that symbolically represents all the programs that match this example. 
However, this time, since $\tool$ has already seen two examples, it tries to search for a program that is consistent with both examples. 
Therefore, it takes the product (intersection) of $\progset_1$ and $\progset_2$, and picks a program out of the product, say $\getcell(\inputcell, \updir, 1, \lambda\startcell.\lambda\itercell. \valneqconst{\itercell}{\missing})$. 

Applying this program to the missing cells in the table, $\david$ managed to fill all of them except $(1,3), (2,3), (1,4)$. 


\underline{\textit{Iteration $3$:}}
$\david$ gave the third example equation, say, $(1,3) \assign \texttt{ID}((3,3))$, which is translated into $(1,3) \mapsto (3,3)$ as the example for the data extraction task. 
$\tool$ repeats the process above to construct an automaton $\progset_3$ and computes the product of $\progset_1, \progset_2$ and $\progset_3$, however, the product becomes empty since there is no conditional-free program in the $\dsl$ that can match all three examples. 

For this case, $\tool$ tries to learn a $\seqconstruct$ program with two branches. 
It first enumerates all possible ways to partition the three examples into two branches. For each partition scheme, it learns a conditional-free program for each branch, using not only the (positive) examples belonging to that branch but also the (negative) examples from the other branch. 
In particular, consider the partition scheme where it puts two examples $(5,3) \mapsto (4,3)$, $(7,5) \mapsto (5,5)$ in the first branch, and puts the other example $(1,3) \mapsto (3,3)$ in the second branch. 
$\tool$ needs to learn a conditional-free program $p_1$ for the first branch that matches both examples in that branch, however, $p_1$ should also not ``match'' the example in the second branch. More specifically, we should have $p_1((5,3)) = (4,3), p_1((7,5)) = (5,5)$ and $p_1((1,3)) = \bottom$ (recall the semantics of a $\seqconstruct$ program). 
After learning $p_1$ for the first branch, $\tool$ continues to learn a conditional-free program $p_2$ for the second branch, using only the (positive) example $(1,3) \mapsto (3,3)$ in that branch, since there are only two branches in the $\seqconstruct$ program. 
$\tool$ repeats this process for all partition schemes, and returns the ``simplest'' $\seqconstruct$ program to $\david$, say, $\seqconstruct(\getcell(\inputcell, \updir, 1, \lambda\startcell.\lambda\itercell.\valneqconst{\itercell}{\missing}), \getcell(\inputcell, \downdir, 1, \lambda\startcell.\lambda\itercell.\valneqconst{\itercell}{\missing}))$. 

$\david$ applied this program to all the missing cells in the table, and got the desired results. 

\subsection{Generalizations}

We summarize several key components in the synthesis process for the simple example in \exref{locfseq}. 
\begin{itemize}
\item 
Translating an example equation into input-output examples for the data extraction task. Since this can be easily supported, we skip the discussion of this in the paper. 
\item 
Representing conditional-free programs. In particular, it represents the program set as an automaton. 
\item 
Manipulating program sets, such as computing their intersection (to handle multiple examples) and selecting the ``best'' program. In particular, it computes the product of automata and selects the ``best'' program by computing the shortest path (``simplest'' program) in an automaton. 
\item 
Learning conditional programs. In particular, it needs an algorithm that enumerates all possible partition schemes, and an algorithm that learns the conditional-free program for each branch using both positive and negative examples for a given partition scheme. 
\end{itemize}



However, the strategy above has some problems and we need to make the following generalizations in order to support learning programs in the full $\dsl$. 
\begin{itemize}
\item 
A automaton is not expressive enough for representing the simple programs in the $\dsl$. 
In particular, an automaton can only represent $\unionconstruct$ programs with one cell, since an accepted string reaches only one final state. It is not able to represent a $\unionconstruct$ program with multiple cells or any $\filterconstruct$ program. 

Essentially, a desirable representation should be able to express the notion of a path reaching potentially multiple final states at a time, instead of reaching only one final state. 
We generalize the representation from an automaton to a hypergraph automaton in order to support this. 
\item 
We define the product of two hypergraph automata in our setting, as well as generalize the selection of programs by finding the shortest path in an automaton to finding the shortest B-path in a hypergraph automaton. 
\end{itemize}


In the following sections, we first present the synthesis algorithm for learning conditional programs, assuming a desirable representation is used. 
Then, we present the representation and its operations, as well as the construction of such a representation from an example. 


==> prose.tex <==
\section{Comparison with PROSE}

In this section, we present a more detailed comparison between the techniques used in \tool and \prose. 
We first explain the conceptual differences between the two techniques. 
Then, we compare them empirically based on the experimental results. 
Finally, we present some insights of our FTA method in the background of version space learning. 

\subsection{Conceptual comparison}




\tool differs from \prose in two aspects: 1) \tool constructs FTA in a forward manner whereas \prose generates the VSA by performing backpropagation, and 2) \tool uses a finite tree automata (FTA) to represent all consistent programs as opposed to the VSA method used in \prose. 


\begin{wrapfigure}{r}{0.45\linewidth}
\begin{minipage}{\linewidth}
\vspace{-20pt}
\small
$\begin{array}{lll}
\langtext{Cell prog.} ~ \cellprog & \assign & \inputcell ~~ | ~~ \getcell(\cellprog, \dir, k, \lambda \startcell. \lambda \itercell. \true) ~; \\ 
\langtext{Direction} ~ \dir & \assign & \updir ~ | ~ \downdir ~ | ~ \leftdir ~ | ~ \rightdir ~; \\ 
\langtext{int} ~ k & \assign & 1 ~ | ~ 2 ~; \\ 
\end{array}$
\caption{A simple syntax of the DSL.}
\figlabel{simplesyntax}
\vspace{10pt}
\end{minipage}
\begin{minipage}{\linewidth}
\small
$\begin{array}{lll}
\langtext{Cell prog.} ~ \cellprog & \assign & \cellprog_3 ~~ | ~~ \cellprog_2 ~~ | ~~ \cellprog_1 ~; \\ 
\langtext{Cell prog.} ~ \cellprog_3 & \assign & \getcell(\cellprog_2, \dir, 1, \lambda \startcell. \lambda \itercell. \true) ~; \\ 
\langtext{Cell prog.} ~ \cellprog_2 & \assign & \getcell(\cellprog_1, \dir, 1, \lambda \startcell. \lambda \itercell. \true) ~; \\ 
\langtext{Cell prog.} ~ \cellprog_1 & \assign & \inputcell ~; \\ 
\langtext{Direction} ~ \dir & \assign & \updir ~ | ~ \downdir ~ | ~ \leftdir ~ | ~ \rightdir ~; \\ 
\langtext{int} ~ k & \assign & 1 ~ | ~ 2 ~; \\ 
\end{array}$
\caption{The unrolled syntax in \prose.}
\figlabel{unrolled}
\end{minipage}
\vspace{-10pt}
\end{wrapfigure}



Let us use the simple example shown in~\exref{exfta} to explain these differences in more details. 
Consider a simple grammar shown in~\figref{simplesyntax}. 
Here, the top-level construct in the DSL is a $\getcell$ operator whose arguments are chosen from a restricted space. 
We assume at most 2 $\getcell$ programs can be nested together. 




\prose first unrolls the grammar to explicitly enforce a hierarchical structure in the grammar. The unrolled grammar is shown in~\figref{unrolled}. 


Then, \prose propagates the specification backwards to generate specifications for smaller sub-expressions by using witness functions.\footnote{A witness function for an expression $e$ is essentially a function that encodes the inverse semantics of $e$, i.e., the inverse $e^{-1}$ of $e$.} 
In this case, the specification for $\cellprog_3$, i.e., $\{ (2,2) \mapsto [ (1,2) ] \}$, is transformed into the specification for $\cellprog_2$, which is $\{ (2,2) \mapsto [ (1,1) ] \} \disj \{ (2,2) \mapsto [ (1,2) ] \disj \{ (2,2) \mapsto [ (2,2) ] \}$. This is because we have $\bigcup_{\dir, k}\getcell^{-1}((1,2), \dir, k, \lambda \startcell. \lambda \itercell. \true) = \{ (1,1), (1,2), (2,2) \}$. \prose does so until it reaches the bottom construct in the grammar, i.e., the constants. 



After the backpropagation finishes, \prose constructs a VSA that represents all the programs it has traversed. \figref{vsafta} (a) shows a part of the whole constructed VSA. As we can see, there is a clear hierarchy in the VSA, and the nodes at the same level are shared. 


\begin{figure*}
\begin{tabular}{c c}
\begin{minipage}{0.5\linewidth}
\centering
\includegraphics[scale=0.42]{figs/simpleVSA}
\end{minipage}
&
\begin{minipage}{0.35\linewidth}
\centering
\includegraphics[scale=0.31]{figs/simpleFTA}
\end{minipage}
\\ \\ 
(a) & (b) \\
\end{tabular}
\caption{(a). Illustration of the construction of VSA in \prose for \exref{exfta} using the grammar in \figref{unrolled}. (b). Illustration of the construction of FTA in \tool for \exref{exfta} using the grammar in \figref{unrolled}.}
\figlabel{vsafta}
\end{figure*}






\subsection{Empirical comparison}


